Are You Smarter Than a Random Expert? The Robust Aggregation of Substitutable Signals

The problem of aggregating expert forecasts is ubiquitous in fields as wide-ranging as machine learning, economics, climate science, and national security. Despite this, our theoretical understanding of this question is fairly shallow. This paper initiates the study of forecast aggregation in a context where experts' knowledge is chosen adversarially from a broad class of information structures. While in full generality it is impossible to achieve a nontrivial performance guarantee, we show that doing so is possible under a condition on the experts' information structure that we call \emph{projective substitutes}. The projective substitutes condition is a notion of informational substitutes: that there are diminishing marginal returns to learning the experts' signals. We show that under the projective substitutes condition, taking the average of the experts' forecasts improves substantially upon the strategy of trusting a random expert. We then consider a more permissive setting, in which the aggregator has access to the prior. We show that by averaging the experts' forecasts and then \emph{extremizing} the average by moving it away from the prior by a constant factor, the aggregator's performance guarantee is substantially better than is possible without knowledge of the prior. Our results give a theoretical grounding to past empirical research on extremization and help give guidance on the appropriate amount to extremize.

==> Conclusion.tex <==
\section{Conclusion}
The results of the previous two sections give a few obvious directions for future work. One is to close one of the (asymptotic) gaps between our positive and negative results. Another is to prove a nontrivial, unconditional negative result in the known prior setting for more than two experts. A third is to search for an aggregation strategy in the known prior setting that outperforms what can be accomplished by the approach of averaging and extremizing by a constant. In particular, \cite{bmtsu14} argues that more extremization is called for when experts' information sets overlap minimally, an observation validated empirically in \cite{su15}. (This is borne out in some of our examples as well: compare information structures $\mathcal{I}_{\text{ind}}$ and $\mathcal{I}_{\text{dep}}$ from Theorem~\ref{thm:known_prior_conditional_negative}.) Although the aggregator does not explicitly know the amount of overlap in the experts' knowledge, the above heuristic can be operationalized by taking the spread of the experts' reports into account: the lower the spread, the more overlap there is likely to be, the less it makes sense to extremize.\\

However, the space of possible directions for exploration extends well beyond closing these gaps. The question ``What approximation ratio is attainable by an aggregation strategy for an adversarially chosen information structure?" can be asked under a variety of settings and conditions. For example:
\begin{itemize}
	\item One can place other conditions on the information structure --- other notions of informational substitutes, or perhaps altogether different assumptions.
	\item While the prior-free and known prior settings are natural starting points, one can consider giving the aggregator more information still (as we briefly touched on in Remark~\ref{rem:other_information}).
	\item While squared loss in a natural choice for the measure of error, other choices may make more sense depending on context. For example, if the forecasters are estimating a probability, it may make sense to judge the aggregator's output based on the KL divergence from the correct answer to the output. This has the benefit of penalizing the aggregator more for e.g. reporting 0.001\% when the right answer is 1\% than for reporting 50\% when the right answer is 51\%.
\end{itemize}

We hope that this work will inspire further exploration of this space, along the three dimensions listed above as well as along dimensions that we have not yet anticipated.
